Enhancing VQE Convergence for Optimization Problems with Problem-specific Parameterized Quantum Circuits

The Variational Quantum Eigensolver (VQE) algorithm is gaining interest for its potential use in near-term quantum devices. In the VQE algorithm, parameterized quantum circuits (PQCs) are employed to prepare quantum states, which are then utilized to compute the expectation value of a given Hamiltonian. Designing efficient PQCs is crucial for improving convergence speed. In this study, we introduce problem-specific PQCs tailored for optimization problems by dynamically generating PQCs that incorporate problem constraints. This approach reduces a search space by focusing on unitary transformations that benefit the VQE algorithm, and accelerate convergence. Our experimental results demonstrate that the convergence speed of our proposed PQCs outperforms state-of-the-art PQCs, highlighting the potential of problem-specific PQCs in optimization problems.

==> tsp_case_study_2to4.tex <==
\subsubsection{PQCs satisfying an L-shaped constraint with CNOT operations}\label{sec:tsp_proposed_2}
For the second PQC, we take into account not only the first line but also taking into account constraint $\sum^{N}_{p=1}x_{1,p} = 1$ in the second line of the constraints of Eq. \ref{eq:tsp} to further reduce the search space, as is shown in Figure \ref{fig:tsp_constraint_fig} (b).
Unlike the first PQC, the situation requires more ``correlations'' among qubits being mapped from variables, since variables $x_{1,p},\; p=1\ldots N$ appear in both the first and the second line; it is no longer possible to realize the constraints by a tensor product of $N$ quantum states.
Hence, we utilize CNOT gates together with the parameterized W state gates to create such a quantum circuit. 

\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.4]{fig/tsp_constraint_figure.pdf}
	\caption{Schematic of the constraints considered for each case; (a) only the first line, (b) a constraint in the second line as well as the first line and (c) all constraints. The blue box represents a constraint in the first line, while the red box indicates a constraint in the second line of constraints of Eq. \ref{eq:tsp}.}
	\label{fig:tsp_constraint_fig}
\end{figure}
The protocol of creating the PQC follows two steps.
First, we construct a quantum circuit satisfying both two constraints,
$\sum^{N}_{p=1}x_{1,p} = 1$ and $\sum^{N}_{v=1}x_{v,1} = 1$, which we call "an L-shaped constraint" because the involved variables form L-shape in Figure \ref{fig:tsp_constraint_fig} (b).
In the L-shaped constraint, one variable in each set of $\{x_{1,p'}|p'=2\ldots N\}$ and $\{x_{v',1}|v'=2\ldots N\}$ has to be one if $x_{1,1}$ is zero, while all variables in $\{x_{1,p'}|p'=2\ldots N\}$ and $\{x_{v',1}|v'=2\ldots N\}$ are zeros if $x_{1,1}$ is one.
According to this, one can easily understand that the corresponding unitary operations on the initialized qubits $q_{i,j}$ being mapped from variables $x_{i,j}$ is realized by applying parameterized W state gates to each set of qubits $\{q_{1,p'}|p'=2\ldots N\}$ and $\{q_{v',1}|v'=2\ldots N\}$ if $\ket{0}_{q_{1,1}}$, and applying identity gates if $\ket{1}_{q_{1,1}}$.
Thus, the PQC can be created with CNOT gates and parameterized W state gates, as depicted in Figure \ref{fig:qc_model2} (a).
In a quantum circuit of Figure \ref{fig:qc_model2} (a), the leftmost $R_{y}$ gate with the trainable parameter $\phi_{0}$ and the following two CNOT gates, $CNOT_{q_{1,1},q_{1,2}}$ and $CNOT_{q_{1,1},q_{2,1}}$, determine whether $\ket{0}_{q_{1,1}}$ or $\ket{1}_{q_{1,1}}$, and whether W state gates or identity gates are applied to each set of qubits $\{q_{1,p'}|p'=2\ldots N\}$ and $\{q_{v',1}|v'=2\ldots N\}$ depending on the condition of $q_{1,1}$, respectively.
Note that we here use the fact that a parameterized W state gate is exactly an identity gate if an X gate is applied to the first qubits beforehand, which can be checked readily by looking into Fig.~\ref{fig:w3_circuit}.
As a result, the quantum circuit can create the desired quantum state expressed as  
\begin{equation}
\label{eq:state_lshape}
\begin{split}
    \cos{\frac{\phi_{0}}{2}} \ket{0}_{q_{1,1}}\ket{W(\phi_{p'})}_{\{q_{1,p'}|p'=2\ldots N\}}\ket{W(\phi_{v'})}_{\{q_{v',1}|v'=2\ldots N\}} \\
    + \sin{\frac{\phi_{0}}{2}} \ket{1}_{q_{1,1}}\ket{0}^{\otimes n-1}_{\{q_{1,p'}|p'=2\ldots N\}}\ket{0}^{\otimes n-1}_{\{q_{v',1}|v'=2\ldots N\}},
\end{split}
\end{equation}
where $\phi$s are all trainable parameters. 

\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.32]{fig/tsp_qc_model1.pdf}
	\caption{A PQC for the second case; (a) a quantum circuit for an L-shaped constraint, (b) a quantum circuit corresponding to the constraint, $\sum^{N}_{v=1}x_{v,p'} = 1$ and (c) a whole picture of the PQC for the second case.}
	\label{fig:qc_model2}
\end{figure}

Second, we apply unitary operations for the remaining constraints, $\sum^{N}_{v=1}x_{v,p'} = 1,\quad p'=2\ldots N$, to a resultant quantum state in Eq. \ref{eq:state_lshape}.
Here, since the qubits corresponding to the variables $\{x_{1,p'}|p'=2\ldots N\}$ in the constraints have already been determined, the constraints can be read in the similar way to the first step as follows; if $x_{1,p'}$ is one, all variables $\{x_{v',p'}|v'=2\ldots N\}$ are zeros, while if $x_{1,p'}$ is zero one variable in $\{x_{v',p'}|v'=2\ldots N\}$ has to be one.
As we have seen in the first step, the corresponding unitary operation can be realized by a $CNOT_{q_{1,p'},q_{2,p'}}$ gate followed by parameterized W state gates on the set of qubits $\{q_{v',p'}|v=2\ldots N\}$ as represented in Figure \ref{fig:qc_model2} (b).
Thus, using $N-1$ \textit{CNOT} gates and $N-1$ circuits for parameterized W sates, we can create the unitary operators that create a quantum state satisfying the remaining constraints.

Following the above two steps, we can create the problem-specific PQC in Figure \ref{fig:qc_model2} (c).  


\subsubsection{PQCs satisfying an L-shaped constraint with parameter sharing }\label{sec:tsp_proposed_3}
For the third PQC, we modify the second PQC to reduce the cost of the implementation for the current quantum processors \cite{preskillNISQ}. 
Since current noisy devices suffer from an exponential decay of quantum coherence, deep circuits would be problematic.
In the second case, the circuit becomes deep due to the dependence in its own structure; firstly, a quantum circuit for an L-shaped constraint is constructed, and then other gates are applied for the remaining constraints.

To remedy this issue, we introduce the technique, \textit{parameter sharing}, which makes the circuit shallower with fewer CNOT gates.
The main point of this technique is as follows; CNOT gates (and also X gates in parameterized W state gates) used in Fig.~\ref{fig:tsp_constraint_fig}
 are replaced with $R_{y}$ gates with the shared parameters such that the probability of obtaining $\ket{1}_{q_{1,p'}}$ is equal to that of $\ket{0}^{\otimes N-1}_{\{q_{v',p'}|v'=2\ldots N\}}$.
To demonstrate the parameter sharing in detail, we provide a simple example of the quantum circuit with $N=3$ in Figure \ref{fig:qc_model3}.
In this scenario, parameters $\phi_{0}$ and $\phi_{2}$ are used for not only $q_{1,1}$ and $q_{1,2}$, but also $q_{2,2}$ and $q_{3,2}$ in unique ways such as $2\arccos{\left(\cos{\phi_{0}/2}\cos{\phi_{2}}\right)}$.
Indeed, the trigonometric functions inside the inverse trigonometric function, $\cos{\phi_{0}/2}\cos{\phi_{2}}$ and $-\cos{\phi_{0}/2}\sin{\phi_{2}}$ are the amplitudes of $\ket{1}_{q_{1,2}}$ and $\ket{1}_{q_{1,3}}$, respectively.
Therefore, the amplitude of $\ket{00}_{\{q_{v,2}|v=2,3\}}$ is always the same as that of $\ket{1}_{q_{1,2}}$ by the parameter sharing (similarly, this is true to $q_{1,3}$, $q_{2,3}$, and $q_{3,3}$).
Note that this technique can be easily extended for PQCs with arbitrary $N$ since the probability of obtaining $\ket{1}_{q_{1,p'}}$ for all $p'=2\ldots N$ is analytically calculated in the similar way as shown in Eq.\eqref{eq:pw_state_final}.

By utilizing such ``classical correlation'', we can create a shallower PQC satisfying the constraints in Figure \ref{fig:tsp_constraint_fig} (b), which is expected to be more suitable for current noisy devices.
However, the technique has a limitation on the ability to restrict the set of bases compared to the second case.
As we can see in Figure \ref{fig:qc_model3}, the quantum state created by the PQC is not fully entangled, i.e. it can be written as the tensor product of small quantum states.
Consequently, the set of the bases of the quantum state includes the bases that are not in the second case. However, the probability to obtain such extra bases is at most a half. This characteristic contributes to interesting results which we will discuss in Sec.~\ref{sec:experiment}

\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.32]{fig/tsp_qc_model2.pdf}
	\caption{A PQC with $N=3$ for the third case. To create the PQC, the top-left circuit appearing in the quantum circuit of the second case is replaced with the top-right circuit.}
	\label{fig:qc_model3}
\end{figure}

\subsubsection{PQCs satisfying all constraints}\label{sec:tsp_proposed_4}
For the fourth PQC, we consider all constraints of Eq. \ref{eq:tsp} to completely exclude the infeasible answers as shown in Fig.~\ref{fig:tsp_constraint_fig} (c). Thus, the set of the bases of the quantum states includes only feasible answers , i.e.  $\mathbb{S}_{\textit{case 4}} = \mathbb{S}_{\textit{feasible}}$.

Such a PQC for arbitrary $N$ can be constructed in a recursive manner. 
After a quantum circuit with $N=2$ is exemplified, we will demonstrate that the PQC with $N=k$ can be constructed using the quantum circuit with $N=k-1$.
The basic idea is that the assignments of feasible answers on the 2D grid as shown in Fig.~\ref{fig:tsp_constraint_fig} (c) can be interpreted as permutation matrices. It is due to the fact that the constraints of Eq.\eqref{eq:tsp} are exactly the same as the definition of permutation matrices.
Note that a permutation matrix is a square matrix, every row and column of which has only one entry, 1 while the other entries are 0.
Hence, with the equivalence of permutation matrices and the assignment of the feasible answers on the 2D grid, we construct the quantum circuit. 

Firstly, we show the PQC with $N=2$.
For the number of city $N=2$, two feasible answers exist, as there are two $2\times 2$ permutation matrices, 
$\left[
    \begin{array}{cc}
      1 & 0  \\
      0 & 1  \\
    \end{array}
  \right]$ 
and
$\left[
    \begin{array}{cc}
      0 & 1  \\
      1 & 0  \\
    \end{array}
  \right]$.
Thus, a quantum state we want to create can be described by the superposition of two bases, $\ket{0110}$ and $\ket{1001}$ with the order of qubits $\ket{q_{1,1}q_{2,1}q_{1,2}q_{2,2}}$. 
A quantum circuit for $N=2$ can be created as shown in Fig.~\ref{fig:qc_model4_neq2}, where the quantum state is represented as $\cos{\phi} \ket{1001} - \sin{\phi} \ket{0110}$.

\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.35]{fig/tsp_qc_cswap_neq2.pdf}
	\caption{A PQC with $N=2$ for the fourth case.}
	\label{fig:qc_model4_neq2}
\end{figure}
Secondly, we show that the PQCs with $N=k$ can be constructed by using the quantum circuit with $N=k-1$. The conceptual overview to create PQCs for the forth case is as shown in Fig.~\ref{fig:qc_model4_concept}.
\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.35]{fig/tsp_cswap_concept.pdf}
	\caption{The conceptual overview to create PQCs for the forth case. (a) illustrates the property of permutation matrices, which is used for constructing PQCs. (b) is a schematic view to create the desired quantum state for $N=k$ by using a quantum state for $N=k-1$.}
	\label{fig:qc_model4_concept}
\end{figure}

Suppose that we have all the permutation matrices of size $k-1$, so the total number of the permutation matrices is $(k-1)!$.
Then one can obtain $k!$ permutation matrices of size $k$ in the following way.
\begin{enumerate}
    \item Pad the additional zeros to all the $(k-1)\times (k-1) $ permutation matrices to form $k\times k$ square matrices.
    \item Set the top right element in each of the matrices as 1 to make them permutation matrices.
    \item Permute the $k$-th and the $j$-th column of the matrices for all $j=1\ldots k-1$.
\end{enumerate}
Note that we here use the fact that exchanging the $i$-th and the $j$-th column of a permutation matrix results in also a permutation matrix.
Consequently, with $(k-1)!$ permutation matrices in the second step and $k(k-1)!$ permutation matrices in the third step, we can obtain $k!$ permutation matrices of size $k$ by the above steps.
In analogous to the case of permutation matrices, we construct a quantum circuit with $N=k$.
Let $\ket{\Psi_{k-1}}$ be a quantum state whose bases are all feasible answers for $N=k-1$ with the order of qubits $\ket{q_{1,1\ldots} q_{1,k-1}q_{2,1}\ldots q_{2,k-1}\ldots q_{k-1,1}\ldots q_{k-1,k-1}}$.
Then, in a similar way, we can create the desired quantum states as follows;
\begin{enumerate}
    \item Prepare the initialized $2k-1$ qubits, labeled as $q_{k,p'}, p'=2\ldots k$ and $q_{v,k},v=1\ldots k$.
    \item Apply a parameterized W state gate to the set of qubits, $\{q_{v,k}|v=1\ldots k\}$.
    \item Apply \textit{CSWAP} gates to the corresponding qubits in $\ket{\Psi_{k-1}}$, $\ket{W_{k}(\psi)}_{\{q_{v,k}|v=1\ldots k\}}$, and $\ket{0}^{\otimes k-1}_{\{q_{k,p'}|p'=1\ldots k-1\}}$; the set of \textit{CSWAP} operations, $\{\textit{CSWAP}_{q_{v',k},q_{k,p'},q_{v',p'}}|p'=1\ldots k-1\}$ are applied for all $v'=1\ldots k-1$.
\end{enumerate}
In this procedure, the parameterized W state gate is used to represent the additional $k$-th row of $k\times k$ matrix, which can be regarded as the permutation inside the $k$-th row. 
Then, \textit{CSWAP} gates are used to serve as the permutation of the remaining rows depending on the state of $k$-th row; the states of $\{q_{k,p'}|p'=1\ldots k-1\}$ and $\{q_{v,p'}|p'=1\ldots k-1\}$ are exchanged if $\ket{1}_{q_{v,k}}$, while the states of $\{q_{k,p'}|p'=1\ldots k-1\}$ and $\{q_{v,p'}|p'=1\ldots k-1\}$ remain unchanged if $\ket{0}_{q_{p,k}}$.
As a demonstration, we give a simple example of the PQC with $N=3$ for the forth case as shown in Fig.~\ref{fig:qc_model4_neq3}.
\begin{figure}[tbp]
	\centering
	\includegraphics[scale=0.3]{fig/tsp_qc_cswap_neq3.pdf}
	\caption{A PQC with $N=3$ for the fourth case.}
	\label{fig:qc_model4_neq3}
\end{figure}

Then the corresponding quantum state is represented as Eq.\eqref{eq:state_proposed4_n_3}, with the order of qubits $\ket{q_{1,1}q_{2,1}q_{3,1}q_{1,2}q_{2,2}q_{3,2}q_{1,3}q_{2,3}q_{3,3}}$, which is exactly the superposition of bases of six feasible answers. 
\begin{equation}
\label{eq:state_proposed4_n_3}
\begin{split}
    \ket{\Psi_{k-1}}=-\cos{\phi_{0}}\sin{\phi_{1}}\cos{\phi_{2}}\ket{100001010}\\
    +\cos{\phi_{0}}\sin{\phi_{1}}\sin{\phi_{2}}\ket{001100010}\\
    +\cos{\phi_{0}}\sin{\phi_{1}}\sin{\phi_{2}}\ket{100010001}\\
    -\sin{\phi_{0}}\sin{\phi_{1}}\cos{\phi_{2}}\ket{010100001} \\
    +\cos{\phi_{0}}\cos{\phi_{1}}\ket{001010100}\\
    -\sin{\phi_{0}}\cos{\phi_{1}}\ket{010001100}
\end{split}
\end{equation}
Therefore, we can construct the PQC for arbitrary $N$ by recursively performing the procedure explained in the above starting from the quantum circuit with $N=2$.






























